Joint functional calculus in algebra of polynomial tempered distributions

In this paper we develop a functional calculus for a countable system of generators of contraction strongly continuous semigroups. As a symbol class of such calculus we use the algebra of polynomial tempered distributions. We prove a differential property of constructed calculus and describe its image with the help of the commutant of polynomial shift semigroup. As an application, we consider a function of countable set of second derivative operators.

==> jinfo.tex <==
\jvolume{22}
\jyear{2016}
\jnumber{1}

